Stochastic Multi-Robot Monitoring on Graphs under Markovian Mobility

We study a stochastic multi-robot monitoring problem on a connected graph $G=(V,E)$, where each robot moves according to a Markov chain on $G$ and monitors the closed neighborhood of its current vertex. The performance of $r$ robots is evaluated in steady state via two objectives: average-case coverage (the expected number of covered vertices) and worst-case coverage (the minimum coverage probability over all vertices). We consider three models: independent homogeneous strategies, where all robots share the same stationary distribution; independent heterogeneous strategies, where robots use different stationary distributions; and centralized strategies, allowing arbitrary correlations between robot locations. For the heterogeneous model, we prove that maximizing average coverage is NP-hard even for two robots, and that replicating an easy-to-compute optimal homogeneous strategy yields a \(\left(1-\left(1-\frac{1}{r}\right)^r\right)\)-approximation for both objective functions in the heterogeneous setting; moreover, no polynomial-time algorithm can achieve a ratio better than \(1-\nicefrac{1}{e}\) unless \(\text{P}=\text{NP}\). Centralized strategies can exploit correlations to reduce redundancy. We develop a hierarchy of approximation factors: for any positive integer \(r'\le r\), writing \(r=hr'+b\) with \(0\le b<r'\), block coordination yields a \(1-\left(1-\frac{r'}{r}\right)^h\left(1-\frac{b}{r}\right)\) approximation for both objectives. We also establish NP-hardness and a tight \(1-\nicefrac{1}{e}\) inapproximability bound. Moreover, we prove diminishing-returns properties with respect to the number of robots: a non-increasing-ratio property holds for the average-case objective in all settings, but not for the heterogeneous worst-case objective.

==> lipics/packages.tex <==
%!TEX root=./main.tex

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc} % MUST INSTALL cm-super package, MiKTeX Settings (Admin) > Refresh FNDB, Update Formats

% \usepackage{amsfonts,amsmath,amssymb,amsthm}
\usepackage{babel}
% \usepackage{collect}
\usepackage{xspace}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{nicefrac}
\usetikzlibrary{fit,positioning}
\usetikzlibrary{decorations.pathmorphing}
% \usepackage{environ} %allows to define environments with align, without latex crapping out

% \usepackage{thmtools}
%\usepackage{thm-restate}


\usepackage[bibliography=common]{apxproof} %(conf submission)
% % \usepackage[appendix=strip]{apxproof}  %remove the appendix (camera ready)
%\usepackage[appendix=inline]{apxproof} %content in the main text (arxiv)
\usetikzlibrary{arrows.meta, positioning}

% \renewcommand{\mainbodyrepeatedtheorem}{\textup{\textbf{(*)}}}
% \newtheoremrep{theorem}{Theorem} 
% \newtheoremrep{lemma}{Lemma}
% \newtheoremrep{claim}{Claim}

\makeatletter
\newcommand{\thmToAppendix}[1]{\axp@writesection \immediate\write\axp@proofsfile{\noexpand\csname#1\endcsname*}}
\newcommand{\appendixSubsection}[1]{\axp@writesection \immediate\write\axp@proofsfile{\noexpand\subsection{#1}}}
\makeatother

% Specific order
% \usepackage{algpseudocode}


% cleverref
\crefname{property}{property}{properties}
\crefname{constraint}{constraint}{constraints}


\newcommand{\NewMathVariable}[2]{\DeclareRobustCommand{#1}[0]{\ensuremath{#2}\xspace}}

\NewMathVariable{\Nbb}{\mathbb{N}}
\NewMathVariable{\Qbb}{\mathbb{Q}}
\NewMathVariable{\Rbb}{\mathbb{R}}
\NewMathVariable{\Zbb}{\mathbb{Z}}
\NewMathVariable{\Rnn}{\mathbb{R}_{\geq 0}}
\NewMathVariable{\Znn}{\mathbb{Z}_{\geq 0}}
\NewMathVariable{\Zp}{\mathbb{Z}_{+}}

\newcommand{\tik}{\textcolor{purple}{\checkmark}}
\newcommand{\OPT}{{\operatorname{OPT}}}
\newcommand{\ALG}{{\operatorname{ALG}}}
\newcommand{\LP}{{\operatorname{LP}}}
\newcommand{\N}{{\mathcal{N}}}
%\newcommand{\P}{{\mathcal{P}}}
\newcommand{\cov}{{\mathrm{cov}}}
\newcommand{\het}{{\mathrm{het}}}
\newcommand{\hhom}{{\mathrm{hom}}}
\newcommand{\cent}{{\mathrm{cent}}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\Safety}{{\mathrm{Safety}}}

\usepackage{mathtools}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\brac}{[}{]}
\DeclarePairedDelimiter{\cbrac}{\{}{\}}
\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
\DeclarePairedDelimiter{\restr}{.}{|}
\DeclarePairedDelimiter{\fceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\ffloor}{\lfloor}{\rfloor}




\makeatletter
\newcommand{\authorcommands}[4][blue!80!black]{%
    \expandafter\def\csname#2m\endcsname##1{\marginpar{$\leftarrow$\fbox{#4}}\footnote{$\Rightarrow$~{\sf ##1 --#3}}}
    % \expandafter\def\csname #2 \endcsname##1{\marginpar{$\leftarrow$\fbox{#4}}\footnote{$\Rightarrow$~{\sf ##1 --#3}}}
    \expandafter\def\csname #2\endcsname{\@ifstar{\csname @#2\endcsname}{\csname @@#2\endcsname}}
    \expandafter\def\csname @#2\endcsname##1{\textcolor{#1}{[#3: ##1]}}
    \expandafter\def\csname @@#2\endcsname##1{\par\noindent\textcolor{#1}{#3: ##1}\par}
}
\newcommand{\noauthorcommands}[4][blue!80!black]{%
    \expandafter\def\csname#2m\endcsname##1{}
    \expandafter\def\csname#2\endcsname##1{}
}
\makeatother

\setcounter{topnumber}{1}
\setcounter{totalnumber}{1}
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}



